MultiInstruct: Improving Multi-Modal Zero-Shot Learning via Instruction Tuning

Instruction tuning, a new learning paradigm that fine-tunes pre-trained language models on tasks specified through instructions, has shown promising zero-shot performance on various natural language processing tasks. However, it has yet to be explored for vision and multimodal tasks. In this work, we introduce MUL-TIINSTRUCT, the first multimodal instruction tuning benchmark dataset that consists of 62 diverse multimodal tasks in a unified seq-to-seq format covering 10 broad categories. The tasks are derived from 21 existing open-source datasets and each task is equipped with 5 expert-written instructions. We take OFA as the base pre-trained model for multimodal instruction tuning, and to further improve its zero-shot performance, we explore multiple transfer learning strategies to leverage the large-scale NATURAL INSTRUCTIONS dataset. Experimental results demonstrate strong zero-shot performance on various unseen multimodal tasks and the benefit of transfer learning from a text-only instruction dataset. We also design a new evaluation metric - Sensitivity, to evaluate how sensitive the model is to the variety of instructions. Our results indicate that fine-tuning the model on a diverse set of tasks and instructions leads to a reduced sensitivity to variations in instructions for each task.

==> figures/num_instruct_results.tex <==
\begin{figure}[tbh!]
    \centering
\includegraphics[width=\columnwidth]{figures/num_instruct_tasks.png}
    \caption{\textbf{The Effect of Variety of Instructions.} \lifu{add the result of OFA based on one instruction} \lifu{add label for y axis}}
    \label{fig:num_instruct_tasks}
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\E}{\mathbb{E}}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/2.5_background.tex <==
\section{Background}

\subsection{Instruction Tuning}
FLAN \cite{wei2021flan} proposed an instruction-based approach for improving the zero-shot learning abilities of language models. In instruction tuning, given the pre-trained language model $M$, we finetune the model $M$ on a collection of tasks $T$ described by instructions. Particular, for each task $t \sim T$ and its associated dataset $\mathcal D^t=\{(x^t_j, y^t_j) \in \mathcal X^t \times \mathcal Y^t\}_{j=1}^N$, we can construct a set of possible instructions $I^t$. During fine-tuning, the input to model $M$ is formatted as the combination of the original input $x^t_j$ and the instruction $i^t \in I^t$. Here, the instruction can consist of the meta information of the task such as task definition, classification options and so on \cite{prakhar2022instructdial}.

\subsection{OFA}

OFA (One For All) \cite{wang2022unifying} is a unified multimodal pre-trained model that unifies a diverse set of crossmodal and unimodal tasks in a single Transformer-based \cite{vaswani2017attention} sequence-to-sequence framework. 
To achieve the unification in architecture, tasks, and modalities, OFA employs a unified vocabulary for all text and visual tokens, including subwords, image codes, and location tokens.

OFA is capable of performing both understanding and generation tasks with single or multiple modalities and is currently the largest open-source multimodal pretrained model available. In this work, we utilize OFA for investigating the effectiveness of instruction-tuning on generative multimodal pretrained models. \lifu{clarify the difference between OFA and MultiInstruct}



==> sections/4_experimental_setup_old.tex <==
\section{Datasets and Experimental Setups}

\lifu{this whole section will be replaced. You can put some information such as Datasets to the previous section 3}
% \noindent \textbf{Comparison among various tuning methods}
% fine-tuning, instruction tuning, prompt tuning, meta -training for in-context learning


% \subsection{Research Questions}
% \label{sec:rq}

% We design experiments to answer the following research questions:

% \noindent \textbf{(1) Effectiveness of Multi-Instructions:} We compare the zero-shot performance of OFA instruction-tuned on different instruction datasets including Natural-Instructions, Multi-Instructions and a combination of Natural-Instructions and Multi-Instructions.
% \noindent \textbf{(2) Utilization of Natural-Instructions} 


% \noindent \textbf{(3) Impact of Instruct-Adapter} We study the impact of Instruct-Adapter 

% \noindent \textbf{(4) Intra-task Robustness} 

% \noindent \textbf{(5) Number of Multimodal Tasks}

% \noindent \textbf{(6) Number of Instructions}

% \noindent \textbf{How to improve Inter-task Sensitivity?}

% \subsection{Training Datasets}
% \paragraph{Multi-Instructions}

% We present Multi-Instructions, the first multimodal instruction tuning dataset comprising 40 diverse multimodal tasks as discussed in Section \ref{sec:multi_instruct}. Table \ref{tab:mm_instruct} demonstrates the list of multimodal tasks included in the dataset, along with an example instruction for each task.

% \paragraph{Natural-Instructions}

% For the natural language dataset, we directly adopt the Natural Instructions \cite{Swaroop2022naturalinstructions}, a crowdsourced text-only instruction dataset that contains over 850 English-language tasks along with human-authored task instructions.

% \paragraph{Mixed-Instructions}
% To construct the Mixed-Instructions dataset, we combine the instances from both the Multi-Instructions and Natural-Instructions datasets, and randomly shuffle the order of the instances to form the Mixed-Instructions dataset.


\subsection{Evaluation Datasets and Tasks}

\input{tables/unseen_tasks.tex}
% To study the research questions introduced in Section \ref{sec:rq}, 
We evaluate the proposed approaches and the baseline models on seven unseen multimodal tasks in a zero-shot manner.  Table \ref{tab:unseen} shows the list of unseen tasks used for evaluation. These tasks are grouped into three categories: Visual Question Answering, Visual Commonsense Reasoning, and Miscellaneous.

\paragraph{Visual Question Answering}

The Visual Question Answering category consists of three tasks: (1) \textit{Outside Knowledge VQA}: Visual question answering that requires external knowledge (2) \textit{Text VQA}: Visual question answering that requires reading and reasoning about text in the image, and (3) \textit{Grounded Visual Question Answering}: Answering the question by selecting the correct region in the image.


\paragraph{Visual Commonsense Reasoning}
The Visual Commonsense Reasoning category consists of two tasks: (1) \textit{Commonsense VQA}: Visual question answering that requires commonsense reasoning, and (2) \textit{Visual Entailment}: Predicting whether the image semantically entails the text. 

% (2) \textit{Visual Answering Justification}: providing rationale explaining why the answer to the visual question is true,

\paragraph{Miscellaneous}
The Miscellaneous category consists of two tasks: (1) \textit{Visual Text Extraction}: Extracting the text in the given image and (2) \textit{Visual Dialogue}: Visual question answering based on dialogue.

% (2) \textit{Grounded Visual Text Extraction}: extracting the text from the given region in the image. We report the results in Table \ref{table:zs_vte}.

% \subsection{Evaluation Metrics}

% We report the accuracy for classification tasks and ROUGE-L \cite{lin2004rouge} for both classification and generation tasks following \citet{Swaroop2022naturalinstructions} which treats all tasks as text generation problems.



% \subsection{Possible Additional Datasets}
% \cite{Radford2021clip,kornblith2018visionTransferDataset}

\subsection{Baselines}
\paragraph{OFA} Follow previous instruction tuning works~\cite{Swaroop2022naturalinstructions}, we use the pretrained unified model OFA-large as our baseline. OFA-large has 472M parameters and was trained on 8 tasks shown in Table~\ref{tab:ofa_dataset}. As reported in the original paper, the model has demonstrated zero-shot generalizability on unseen multimodal tasks.

\paragraph{OFA + Natural-Instructions} Natural Instructions~\cite{Swaroop2022naturalinstructions}, a crowdsourcing natural language instruction dataset, has shown its great capability to enable the pretrained language models to follow instructions on unseen tasks. Thus, we propose to leverage the Natural Instructions dataset to finetune OFA.

\paragraph{OFA + Multi-Instructions} To see the benefit of our newly introduced multimodal instruction dataset, we perform instruction tuning of the OFA-large model on Multi-Instructions dataset.

\paragraph{OFA + Mixed-Instructions} Perform instruction tuning of the OFA-large model on our mixed dataset multi-instruct dataset.

\subsection{Instruct-Adapter} 
As the proposed Instruct-Adapter and Pre-Instruction Tuning are orthogonal methods, in the experiment we apply Pre-Instruction Tuning to Instruct-Adapter and just call the method Instruct-Adapter. We also provide 3 variants to better understand the performance of Instruct-Adapter when combined with different training datasets. Below "w.o." denotes "with only".

\paragraph{Instruct-Adapter w.o. Natural-Instructions} We only fine-tune the parameters of adapters on Natrual-Instructions.

\paragraph{Instruct-Adapter w.o. Multi-Instructions}  We only fine-tune the parameters of adapters on Multi-Instructions.

\paragraph{Instruct-Adapter w.o. Mix-Instructions} We fine-tune the parameters of adapters on the mixture of Natrual-Instructions and Multi-Instructions.

% \paragraph{Instruct-Adapter + Two-Stage Instruction Tuning} We first fine-tune the adapter parameters on Natural-Instructions and then fine-tune them on Multi-Instructions.

% \paragraph{Instruct-Adapter + Two-Stage Joint Instruction Tuning} We first only fine-tune the adapter parameters on Natural-Instructions. Then, we fine-tune both OFA and adapter parameters on Multi-Instructions.

% \paragraph{OFA + Two-Stage Instruction Tuning} We first perform instruction tuning on the natural instructions dataset, which teaches the model to follow instructions. However, due to the lack of image in the input and output, the pure language instruction tuning can cause the misalignment between the vision architecture and the language architecture in OFA. To align the two parameter space, we further train OFA on our Multi-Instructions dataset. 

% \subsection{Combine Instruction Tuning with Adapter}

\subsection{Training Details}
To construct the training dataset, we select all the English-language tasks from the Natural-Instructions dataset, which consists of 895 tasks and approximately 2.3 million instances. For the Multi-Instructions dataset, we sample a maximum of 10,000 instances per task and obtain a training dataset containing 470,917 instances. During training, each instance is randomly paired with one of five instruction templates based on its task. For OFA and other model variants that were trained only on the Natural-Instructions dataset, we evaluated them on instruction templates that have removed all specific tokens ("[Options]" and "||||") to ensure a fair comparison, as these models have not encountered such specific tokens during fine-tuning. We set the maximum length of input tokens to 1024 and the maximum target length to 512. For image preprocessing, we strictly follow the process in the OFA. Please refer to the original paper for more details. We train the models on 8 Nvidia A100 GPUs with a batch size 8 per GPU, a learning rate of 1e-05, and float16 enabled for 3 epochs for all the setups and datasets.

% \subsection{Implementation Details}

% In our experiments, we use OFA-Huge \cite{wang2022unifying}, a multimodal pretrained model of 930M parameters.





==> tables/unseen_tasks.tex <==
\begin{table}[!bth]
\scriptsize
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|c}
\toprule
Task Name & Dataset & Task Type   \\
\midrule
 % Hateful Content Detection & HatefulMemes & Classification \\
  Commonsense Visual Question Answering & Visual Commonsense Reasoning & Classification \\
  % Answering Justification & Visual Commonsense Reasoning & Classification \\
  Visual Entailment &  SNLI-VE & Classification \\
 % & Private Visual Information Recognition &VizWiz Visual Privacy & Classification \\
 % & (Un)intentional Privacy Leak Recognition &VizWiz Visual Privacy & Classification \\
  % Purpose-driven Affordance Detection & PAD & Classification \\
  Visual Text Extraction & HatefulMemes & Generation\\
  Outside Knowledge VQA & OK-VQA & Generation\\
  Text VQA & TextVQA  & Generation  \\
  % QA Grounded in Text and Image &MuMuQA & Generation \\
  Dialogue Grounded in Vision &VisDial & Generation \\
  Grounded Visual Question Answering  & Visual7W & Generation \\
  % Grounded Visual Text Extraction & OCR & Generation\\
\bottomrule
\end{tabular}
}
\caption{Unseen tasks for evaluation}
\label{tab:unseen}
\end{center}
\end{table}


==> tables/zs_im_gen.tex <==
\begin{table}[!t]
  \centering
  % \scriptsize
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l cccc }
  \toprule
   \multirow{3}{*}{\centering \textbf{Model}} & \multicolumn{4}{c}{\textbf{Descriptive Partial Image Extraction}}\\
   % && \multicolumn{2}{c}{\textbf{Purpose-driven Affordance}} \\
   %
   \cline{2-5}
   % \cline{11-12} 
  %
  & \multicolumn{2}{c}{FID} & \multicolumn{2}{c}{IS}\\
  \cline{2-5} 
  & Max & Avg $\pm$ \text{Std} & Max & Avg $\pm$ \text{Std} \\
  \midrule
  %\rowcolor{Gray} \multicolumn{8}{l}{\textbf{Baselines}} \\
  OFA & \\
  OFA$_\text{MultiInstruct}$ & \\
  \midrule
  \rowcolor{Gray} \multicolumn{5}{l}{\textbf{Transfer Learning from \textsc{Natural Instructions}}} \\
  OFA$_\text{NaturalInstruct}$ & \\
  OFA$_\text{MixedInstruct}$ & \\
  OFA$_\text{SeqInstruct}$ &   \\
  OFA$_\text{AdapterInstruct}$ & \\
  \bottomrule
  \end{tabular}}
  \caption{\textbf{Zero-shot Performance on Multimodal Commonsense Reasoning.} The best performance is in \textbf{bold}.}
  \label{table:zs_im_gen}
  \end{table}  

==> tables/zs_task_clusters.tex <==
\begin{table*}[!t]
  \centering
  % \scriptsize
  \resizebox{0.7\linewidth}{!}{%
  \begin{tabular}{l cccc c cc}
  \toprule
   \multirow{3}{*}{\centering \textbf{Model}} & \multicolumn{4}{c}{\textbf{Commonsense VQA}}  && \multicolumn{2}{c}{\textbf{Visual Entailment}} \\
   % && \multicolumn{2}{c}{\textbf{Purpose-driven Affordance}} \\
   %
   \cline{2-5} \cline{7-8} 
   % \cline{11-12} 
  %
  & \multicolumn{2}{c}{RougeL} & \multicolumn{2}{c}{ACC} && \multicolumn{2}{c}{ACC}\\
  \cline{2-5} \cline{7-8}
  & Max & Avg $\pm$ \text{Std} & Max & Avg $\pm$ \text{Std} && Max & Avg$\pm$ \text{Std}\\
  \midrule
  %\rowcolor{Gray} \multicolumn{8}{l}{\textbf{Baselines}} \\
  OFA & 17.93 & 14.97 $\pm$ 4.30 & 0.73 & 0.40 $\pm$0.29 && 49.99 & 41.86  $\pm$ 10.99\\
  OFA$_\text{MultiInstruct}$ & \textbf{51.23} & \textbf{50.54} $\pm$ 0.66 & 31.91 & \textbf{31.08} $\pm$ 1.05 && \textbf{54.81} & \textbf{54.26} $\pm$ 0.66 \\
  \midrule
  \rowcolor{Gray} \multicolumn{8}{l}{\textbf{Transfer Learning from \textsc{Natural Instructions}}} \\
  OFA$_\text{NaturalInstruct}$ & 27.15 & 14.99 $\pm$ 9.12 & 7.35 & 2.04 $\pm$ 3.01 && 33.28 & 14.86 $\pm$ 16.68  \\
  OFA$_\text{MixedInstruct}$ & 49.95 & 48.77 $\pm$ 1.19 & 30.49 & 29.47 $\pm$ 0.93 && 53.94 & 53.07 $\pm$ 0.99 \\
  OFA$_\text{SeqInstruct}$ & 50.80 & 49.79 $\pm$ 1.31& \textbf{32.00} & 30.86 $\pm$ 1.13   &&52.71 & 51.86 $\pm$ 0.93 \\
  OFA$_\text{AdapterInstruct}$ & 47.64 & 46.36 $\pm$ 1.42 & 26.77 & 25.38 $\pm$ 1.09 && 47.19 & 43.84 $\pm$ 3.82\\
  
  \bottomrule
  \end{tabular}}
  \caption{\textbf{Zero-shot Performance on Multimodal Commonsense Reasoning.} The best performance is in \textbf{bold}.}
  \label{table:zs_vcr}
  \end{table*}  

==> tables/zs_v_domain_specific.tex <==
\begin{table*}[!t]
  \centering
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l cccc c cccc c cc}
  \toprule
   \multirow{3}{*}{\centering \textbf{Model}} & \multicolumn{4}{c}{\textbf{Outside Knowledge VQA}} && \multicolumn{4}{c}{\textbf{Text VQA}} && \multicolumn{2}{c}{\textbf{Grounded VQA}}\\
   %
   \cline{2-5} \cline{7-10} \cline{12-13}
  %
  & \multicolumn{2}{c}{RougeL} & \multicolumn{2}{c}{ACC} && \multicolumn{2}{c}{RougeL} & \multicolumn{2}{c}{ACC}  &&  \multicolumn{2}{c}{ACC} \\
  \cline{2-5} \cline{7-10} \cline{12-13}
  & Max & Avg $\pm$ \text{Std} & Max & Avg $\pm$ \text{Std} && Max & Avg $\pm$ \text{Std} & Max & Avg $\pm$ \text{Std} && Max & Avg $\pm$ \text{Std} \\
  \midrule
  % OFA \\
  % \midrule
  %\rowcolor{Gray} \multicolumn{13}{l}{\textbf{Baselines}} \\
  OFA & 31.54 & 24.13 $\pm$ 10.33 & 28.38 & 21.19 $\pm$ 8.89  && 15.21 & 9.30 $\pm$ 5.42 & 12.32 & 7.96 $\pm$ 4.20  && 0.02 & 0.00 $\pm$ 0.01  \\
  OFA$_\text{MultiInstruct}$ &  32.55 & 30.31 $\pm$ 1.81 & 28.76 & 26.88 $\pm$ 1.63 && \textbf{25.13} & 20.31 $\pm$ 5.75 & \textbf{20.62} & 17.29 $\pm$ 4.31 && 63.85 & 42.03 $\pm$ 29.43 \\
  \midrule
  \rowcolor{Gray} \multicolumn{13}{l}{\textbf{Transfer Learning from \textsc{Natural Instructions}}} \\
  OFA$_\text{NaturalInstruct}$ &  14.51 & 13.82 $\pm$ 0.57 & 12.21 & 11.56 $\pm$ 0.65 && 5.59 & 5.40 $\pm$ 0.24 & 4.18 & 3.78 $\pm$ 0.27  && 0.00 & 0.00 $\pm$ 0.00 \\
  OFA$_\text{MixedInstruct}$ & 32.15 & 30.95 $\pm$ 0.96 & 28.06 & 27.02 $\pm$ 0.71 && 19.07 & 17.37 $\pm$ 1.72 & 15.52 & 14.41 $\pm$ 1.10 && 62.23 & 49.62 $\pm$ 21.55  \\
  OFA$_\text{SeqInstruct}$ & \textbf{32.97} & \textbf{31.70} $\pm$ 1.14 & \textbf{28.91} & \textbf{27.72} $\pm$ 1.04 && 24.76 & \textbf{23.61} $\pm$ 1.37 & 20.48 & \textbf{19.61} $\pm$ 0.93 && \textbf{64.20} & 50.20 $\pm$ 22.56 \\
  OFA$_\text{AdapterInstruct}$ & 30.84& 27.16 $\pm$ 2.98 & 26.91 & 23.16$\pm$ 3.31 && 23.91 & 19.61 $\pm$ 4.33 & 19.56 & 15.90 $\pm$ 3.59  && 63.15 & \textbf{53.51} $\pm$ 16.62 \\
  \bottomrule
  \end{tabular}}
  \caption{\textbf{Zero-shot Performance on Question Answering datasets.} The best performance is underscored
and in bold and the second best is in bold. }
  \label{table:zs_vqa}
  \end{table*}



\begin{table*}[!t]
  \centering
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l cc c ccc c ccc }
  \toprule
   \multirow{2}{*}{\centering \textbf{Model}} & \multicolumn{2}{c}{\textbf{Hateful Content Detection}} && \multicolumn{3}{c}{\textbf{VisDial}} && \multicolumn{3}{c}{\textbf{Multimodal Open-Domain Dialogue}}\\
   %
   \cline{2-3} \cline{5-7} \cline{9-11} 
  %
  & Acc & RougeL  && M & R@1 & RougeL &&  M & R@1 & RougeL \\
  \midrule
  OFA & \\
  \midrule
  {\small \bf OFA} \\
  + Natural-Instructions &  \\
  + Muti-Instructions & \\
  + Mixed-Instructions & \\
  + Two-Stage Instruction Tuning \\
  \midrule
  {\small \bf Instruct-Adapter} \\
  + Natural-Instructions &  \\
  + Muti-Instructions &   \\
  + Mixed-Instructions & \\
  + Two-Stage Instruction Tuning \\
  + Two-Stage Joint Instruction Tuning \\
  \bottomrule
  \end{tabular}}
  \caption{\textbf{Zero-shot Performance on Multimodal Domain Specific Tasks.}}
  \label{table:zs_vqa}
  \end{table*}

==> tables/zs_vcr_bak.tex <==
\begin{table*}[!t]
  \centering
  % \scriptsize
  \resizebox{0.7\linewidth}{!}{%
  \begin{tabular}{l cccc c cc}
  \toprule
   \multirow{3}{*}{\centering \textbf{Model}} & \multicolumn{4}{c}{\textbf{Commonsense VQA}}  && \multicolumn{2}{c}{\textbf{Visual Entailment}} \\
   % && \multicolumn{2}{c}{\textbf{Purpose-driven Affordance}} \\
   %
   \cline{2-5} \cline{7-8} 
   % \cline{11-12} 
  %
  & \multicolumn{2}{c}{RougeL} & \multicolumn{2}{c}{ACC} && \multicolumn{2}{c}{ACC}\\
  \cline{2-5} \cline{7-8}
  & Max & Avg $\pm$ \text{Std} & Max & Avg $\pm$ \text{Std} && Max & Avg$\pm$ \text{Std}\\
  \midrule
  %\rowcolor{Gray} \multicolumn{8}{l}{\textbf{Baselines}} \\
  OFA & 17.93 & 14.97 $\pm$ 4.30 & 0.73 & 0.40 $\pm$0.29 && 49.99 & 41.86  $\pm$ 10.99\\
  OFA$_\text{MultiInstruct}$ & \textbf{51.23} & \textbf{50.54} $\pm$ 0.66 & 31.91 & \textbf{31.08} $\pm$ 1.05 && \textbf{54.81} & \textbf{54.26} $\pm$ 0.66 \\
  \midrule
  \rowcolor{Gray} \multicolumn{8}{l}{\textbf{Transfer Learning from \textsc{Natural Instructions}}} \\
  OFA$_\text{NaturalInstruct}$ & 27.15 & 14.99 $\pm$ 9.12 & 7.35 & 2.04 $\pm$ 3.01 && 33.28 & 14.86 $\pm$ 16.68  \\
  OFA$_\text{MixedInstruct}$ & 49.95 & 48.77 $\pm$ 1.19 & 30.49 & 29.47 $\pm$ 0.93 && 53.94 & 53.07 $\pm$ 0.99 \\
  OFA$_\text{SeqInstruct}$ & 50.80 & 49.79 $\pm$ 1.31& \textbf{32.00} & 30.86 $\pm$ 1.13   &&52.71 & 51.86 $\pm$ 0.93 \\
  OFA$_\text{AdapterInstruct}$ & 47.64 & 46.36 $\pm$ 1.42 & 26.77 & 25.38 $\pm$ 1.09 && 47.19 & 43.84 $\pm$ 3.82\\
  \bottomrule
  \end{tabular}}
  \caption{\textbf{Zero-shot Performance on Multimodal Commonsense Reasoning.} The best performance is in \textbf{bold}.}
  \label{table:zs_vcr}
  \end{table*} 

==> tables/zs_vqa.tex <==
\begin{table*}[!t]
  \centering
  \resizebox{0.62\linewidth}{!}{%
  \begin{tabular}{l cccc c cc}
  \toprule
   \multirow{3}{*}{\centering \textbf{Model}} & \multicolumn{4}{c}{\textbf{Text VQA}} && \multicolumn{2}{c}{\textbf{Grounded VQA}}\\
   %
   \cline{2-5} \cline{7-8}
  %
  &\multicolumn{2}{c}{RougeL} & \multicolumn{2}{c}{ACC}  &&  \multicolumn{2}{c}{ACC} \\
  \cline{2-5} \cline{7-8}
  & Max & Avg $\pm$ \text{Std} & Max & Avg $\pm$ \text{Std} && Max & Avg $\pm$ \text{Std} \\
  \midrule
  % OFA \\
  % \midrule
  %\rowcolor{Gray} \multicolumn{13}{l}{\textbf{Baselines}} \\
  OFA &  15.21 & 9.30 $\pm$ 5.42 & 12.32 & 7.96 $\pm$ 4.20  && 0.02 & 0.00 $\pm$ 0.01  \\
  OFA$_\text{TaskName}$ & 23.80 & - & 20.02 & - && 0.00 & -\\ 
  OFA$_\text{MultiInstruct}$ & \textbf{27.22} & 26.46 $\pm$ 0.83 & \textbf{22.70} & 22.00 $\pm$ 0.70 && \textbf{64.32} & 47.22 $\pm$ 23.08 \\
  \midrule
  \rowcolor{Gray} \multicolumn{8}{l}{\textbf{Transfer Learning from \textsc{Natural Instructions}}} \\
  OFA$_\text{NaturalInstruct}$ & 5.59 & 5.40 $\pm$ 0.24 & 4.18 & 3.78 $\pm$ 0.27  && 0.00 & 0.00 $\pm$ 0.00   \\
  OFA$_\text{MixedInstruct}$ & 24.15 & 23.67 $\pm$ 0.47 & 20.10 & 19.62 $\pm$ 0.46 && 63.79 & \textbf{54.99} $\pm$ 18.16    \\
  OFA$_\text{SeqInstruct}$ & 27.03 & \textbf{26.67} $\pm$ 0.47 & 22.64 & \textbf{22.28} $\pm$ 0.46 && 64.19 & 54.46 $\pm$ 15.96 \\
  % OFA$_\text{AdapterInstruct}$ &  \\
  
  \bottomrule
  \end{tabular}}
  \vspace{-2mm}
  \caption{\textbf{Zero-shot Performance on Question Answering datasets.} The best performance is in \textbf{bold}. 
% \lifu{highlight all the best scores for all the tables}
}
  \label{table:zs_vqa}
  \end{table*}
  


==> tables/zs_vqa_bak.tex <==
\begin{table*}[!t]
  \centering
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l cccc c cccc c cc}
  \toprule
   \multirow{3}{*}{\centering \textbf{Model}} & \multicolumn{4}{c}{\textbf{Outside Knowledge VQA}} && \multicolumn{4}{c}{\textbf{Text VQA}} && \multicolumn{2}{c}{\textbf{Grounded VQA}}\\
   %
   \cline{2-5} \cline{7-10} \cline{12-13}
  %
  & \multicolumn{2}{c}{RougeL} & \multicolumn{2}{c}{ACC} && \multicolumn{2}{c}{RougeL} & \multicolumn{2}{c}{ACC}  &&  \multicolumn{2}{c}{ACC} \\
  \cline{2-5} \cline{7-10} \cline{12-13}
  & Max & Avg $\pm$ \text{Std} & Max & Avg $\pm$ \text{Std} && Max & Avg $\pm$ \text{Std} & Max & Avg $\pm$ \text{Std} && Max & Avg $\pm$ \text{Std} \\
  \midrule
  % OFA \\
  % \midrule
  %\rowcolor{Gray} \multicolumn{13}{l}{\textbf{Baselines}} \\
  OFA & 31.54 & 24.13 $\pm$ 10.33 & 28.38 & 21.19 $\pm$ 8.89  && 15.21 & 9.30 $\pm$ 5.42 & 12.32 & 7.96 $\pm$ 4.20  && 0.02 & 0.00 $\pm$ 0.01  \\
  OFA$_\text{MultiInstruct}$ &  32.55 & 30.31 $\pm$ 1.81 & 28.76 & 26.88 $\pm$ 1.63 && \textbf{25.13} & 20.31 $\pm$ 5.75 & \textbf{20.62} & 17.29 $\pm$ 4.31 && 63.85 & 42.03 $\pm$ 29.43 \\
  \midrule
  \rowcolor{Gray} \multicolumn{13}{l}{\textbf{Transfer Learning from \textsc{Natural Instructions}}} \\
  OFA$_\text{NaturalInstruct}$ &  14.51 & 13.82 $\pm$ 0.57 & 12.21 & 11.56 $\pm$ 0.65 && 5.59 & 5.40 $\pm$ 0.24 & 4.18 & 3.78 $\pm$ 0.27  && 0.00 & 0.00 $\pm$ 0.00 \\
  OFA$_\text{MixedInstruct}$ & 32.15 & 30.95 $\pm$ 0.96 & 28.06 & 27.02 $\pm$ 0.71 && 19.07 & 17.37 $\pm$ 1.72 & 15.52 & 14.41 $\pm$ 1.10 && 62.23 & 49.62 $\pm$ 21.55  \\
  OFA$_\text{SeqInstruct}$ & \textbf{32.97} & \textbf{31.70} $\pm$ 1.14 & \textbf{28.91} & \textbf{27.72} $\pm$ 1.04 && 24.76 & \textbf{23.61} $\pm$ 1.37 & 20.48 & \textbf{19.61} $\pm$ 0.93 && \textbf{64.20} & 50.20 $\pm$ 22.56 \\
  OFA$_\text{AdapterInstruct}$ & 30.84& 27.16 $\pm$ 2.98 & 26.91 & 23.16$\pm$ 3.31 && 23.91 & 19.61 $\pm$ 4.33 & 19.56 & 15.90 $\pm$ 3.59  && 63.15 & \textbf{53.51} $\pm$ 16.62 \\
  % + Natural-Instructions &  14.51 & 13.82 $\pm$ 0.57 & 12.21 & 11.56 $\pm$ 0.65 && 5.59 & 5.40 $\pm$ 0.24 & 4.18 & 3.78 $\pm$ 0.27  && 0.00 & 0.00 $\pm$ 0.00 \\
  % + Muti-Instructions &  32.55 & 30.31 $\pm$ 1.81 & 28.76 & 26.88 $\pm$ 1.63 && \textbf{25.13} & 20.31 $\pm$ 5.75 & \textbf{20.62} & 17.29 $\pm$ 4.31 && 63.85 & 42.03 $\pm$ 29.43 \\
  % + Mixed-Instructions & 32.15 & 30.95 $\pm$ 0.96 & 28.06 & 27.02 $\pm$ 0.71 && 19.07 & 17.37 $\pm$ 1.72 & 15.52 & 14.41 $\pm$ 1.10 && 62.23 & 49.62 $\pm$ 21.55  \\
  % \midrule
  % \rowcolor{Gray} \multicolumn{13}{l}{\textbf{Ours}} \\
  % Pre-Instruction Tuning & \textbf{32.97} & \textbf{31.70} $\pm$ 1.14 & \textbf{28.91} & \textbf{27.72} $\pm$ 1.04 && 24.76 & \textbf{23.61} $\pm$ 1.37 & 20.48 & \textbf{19.61} $\pm$ 0.93 && \textbf{64.20} & 50.20 $\pm$ 22.56 \\
  % Instruct-Adapter & 30.84& 27.16 $\pm$ 2.98 & 26.91 & 23.16$\pm$ 3.31 && 23.91 & 19.61 $\pm$ 4.33 & 19.56 & 15.90 $\pm$ 3.59  && 63.15 & \textbf{53.51} $\pm$ 16.62 \\
  % \midrule
  % \rowcolor{Gray} \multicolumn{13}{l}{\textbf{Ablations}} \\
  % Instruct-Adapter \\
  % w.o. Natural-Instructions & 13.85 & 13.17 $\pm$ 0.62 & 11.77 & 11.05 $\pm$ 0.54 && 6.44 & 5.22 $\pm$ 0.97 & 4.92 & 3.66 $\pm$ 0.99  && 0.00 & 0.00 $\pm$ 0.00 \\
  % w.o. Muti-Instructions & 30.35 & 27.63 $\pm$ 2.43 & 27.21 & 24.79 $\pm$ 2.16 && 24.66 & 16.56 $\pm$ 8.58 & 20.22 & 14.08 $\pm$ 6.78  && 62.46 & 38.42 $\pm$ 31.16\\
  % w.o. Mixed-Instructions & 27.85 & 26.58 $\pm$ 1.11 & 24.61 & 23.19 $\pm$ 1.32 && 7.73 & 6.97 $\pm$ 0.80 & 6.70& 5.72 $\pm$ 0.95 && 57.00 & 43.98 $\pm$ 20.34\\
  % + One-Stage Joint Multi-Instructions & 32.22 & 30.42 $\pm$ 1.46 & 28.72 & \second{27.20} $\pm$ 1.22 && \second{25.06} & 20.55 $\pm$ 5.16 & 20.38 & 17.27 $\pm$ 3.78  && \second{64.79} & 43.49 $\pm$ 28.42 \\
  % + Two-Stage Instruction Tuning   & 30.84& 27.16 $\pm$ 2.98 & 26.91 & 23.16$\pm$ 3.31 && 23.91 & 19.61 $\pm$ 4.33 & 19.56 & 15.90 $\pm$ 3.59  && 63.15 & \first{53.51} $\pm$ 16.62 \\
  % + Two-Stage Joint Instruction Tuning & 32.52 & 30.61$\pm$ 1.44 & 28.72 & 27.09$\pm$ 1.48 && 24.00 & \second{21.88}$\pm$ 1.98 & 19.64 & \second{18.21} $\pm$ 1.37  && \first{64.88} & 47.37 $\pm$ 25.18\\
  % + Two-Stage Joint Instruction Tuning 10 & 32.23 & 30.06 $\pm$ 1.78 & 28.34 & 26.62 $\pm$ 1.70 && 24.39 & 22.04 $\pm$ 2.00 & 20.0 & 18.24 $\pm$ 1.73  && 64.70 & 54.18 $\pm$ 17.67 \\
  
  \bottomrule
  \end{tabular}}
  \caption{\textbf{Zero-shot Performance on Question Answering datasets.} The best performance is underscored
and in bold and the second best is in bold. }
  \label{table:zs_vqa}
  \end{table*}
  
  
% 1. train OFA or not
% 2. train adapter or not
% 3. two stage or not

% Train OFA (vision only)\\
% Train OFA (mix)\\
% Train OFA (two stage)\\
% Freeze OFA, train Adapter (mix)\\
% Freeze OFA, train Adapter (two stage)\\
% Train OFA, train Adapter (mix)\\
% Train OFA, train Adapter (two stage)\\
% Freeze OFA, train Adapter only (stage 1), train OFA+Adapter (stage 2)

% Vision 20
% Vision 40

% Baseline: OFA (unsupervised based on original OFA), OFA (finetuned based on vision 40), OFA+Adapter (finetuned on vision 40), add another two vision-language pretrained models as baselines

  


==> tables/zs_vte_bak.tex <==
\begin{table*}[!t]
  \centering
  \resizebox{0.7\linewidth}{!}{%
  % \tiny
  \begin{tabular}{l cc c cccc}
  \toprule
   \multirow{3}{*}{\centering \textbf{Model}} & \multicolumn{2}{c}{\textbf{Visual Text Extraction}} && \multicolumn{4}{c}{\textbf{Visual Dialogue}}  \\
   %
   \cline{2-3} \cline{5-8}
  %
  & \multicolumn{2}{c}{RougeL} && \multicolumn{2}{c}{RougeL} & \multicolumn{2}{c}{ACC}  \\
  \cline{2-3} \cline{5-8}
  & Max & Avg$\pm$ \text{Std} && Max & Avg $\pm$ \text{Std} & Max & Avg $\pm$ \text{Std}  \\
  \midrule
  %\rowcolor{Gray} \multicolumn{8}{l}{\textbf{Baselines}} \\
  OFA & 36.31 & 17.62 $\pm$ 16.82 && 45.46 & 28.71 $\pm$ 9.81 & 37.63 & 23.97 $\pm$ 8.05\\
OFA$_\text{MultiInstruct}$ & 56.56 & 28.16 $\pm$ 25.62 && \textbf{46.60} & 34.80 $\pm$ 6.61 & \textbf{38.47} & 29.31 $\pm$ 5.13 \\
\midrule
\rowcolor{Gray} \multicolumn{8}{l}{\textbf{Transfer Learning from \textsc{Natural Instructions}}} \\
OFA$_\text{NaturalInstruct}$ &  5.65 & 1.24 $\pm$ 2.48 && 30.94 & 27.91 $\pm$ 2.16 & 25.95 & 23.23 $\pm$ 1.92 \\
OFA$_\text{MixedInstruct}$ & 41.66 & 27.07 $\pm$ 10.13  && 46.01 & 38.49 $\pm$ 4.71 & 37.93 & \textbf{32.16} $\pm$ 3.63 \\
OFA$_\text{SeqInstruct}$ & 57.84 & \textbf{49.16} $\pm$ 10.38  && 46.59 & \textbf{36.50} $\pm$ 6.06 & \textbf{38.47} & 30.69 $\pm$ 4.73\\
OFA$_\text{AdapterInstruct}$ & \textbf{58.11} & 38.38 $\pm$ 23.98&&  46.17 & 31.30 $\pm$ 8.39 & 38.00 & 25.59 $\pm$ 7.06 \\
    
  % + Natural-Instructions &  5.65 & 1.24 $\pm$ 2.48 && 30.94 & 27.91 $\pm$ 2.16 & 25.95 & 23.23 $\pm$ 1.92 \\
  % + Muti-Instructions & 56.56 & 28.16 $\pm$ 25.62 && \textbf{46.60} & 34.80 $\pm$ 6.61 & \textbf{38.47} & 29.31 $\pm$ 5.13 \\
  % + Mixed-Instructions & 41.66 & 27.07 $\pm$ 10.13  && 46.01 & 38.49 $\pm$ 4.71 & 37.93 & \textbf{32.16} $\pm$ 3.63 \\
  % \midrule
  % \rowcolor{Gray} \multicolumn{8}{l}{\textbf{Ours}} \\
  %   Pre-Instruction Tuning & 57.84 & \textbf{49.16} $\pm$ 10.38  && 46.59 & \textbf{36.50} $\pm$ 6.06 & \textbf{38.47} & 30.69 $\pm$ 4.73\\
  %   Instruct-Adapter & \textbf{58.11} & 38.38 $\pm$ 23.98&&  46.17 & 31.30 $\pm$ 8.39 & 38.00 & 25.59 $\pm$ 7.06 \\
  % \midrule
  % \rowcolor{Gray} \multicolumn{8}{l}{\textbf{Ablations}} \\
  % Instruct-Adapter \\
  % w.o. Natural-Instructions & 6.42 & 2.50 $\pm$ 2.75 && 31.59 & 18.83 $\pm$ 7.75 & 26.32 & 15.09 $\pm$ 6.86 \\
  % w.o. Muti-Instructions & 52.29 & 22.92 $\pm$ 21.17 && 46.53 & 31.55 $\pm$ 8.61 & 38.33 & 26.38 $\pm$ 6.90  \\
  % w.o. Mixed-Instructions & 5.52 & 2.60 $\pm$ 1.84&& 44.29 & 29.80 $\pm$ 8.44 & 36.52 & 24.22 $\pm$ 7.14 \\
  % + One-Stage Joint Multi-Instructions & 62.64 & 32.78 $\pm$ 27.36 && 46.70 & 35.07 $\pm$ 6.52 & 38.58 & 29.55 $\pm$ 5.06\\
  % + Two-Stage Instruction Tuning & 58.11 & 38.38 $\pm$ 23.98&&  46.17 & 31.30 $\pm$ 8.39 & 38.00 & 25.59 $\pm$ 7.06 \\
  % + Two-Stage Joint Instruction Tuning &63.36 & 52.04 $\pm$ 12.22 && 46.52 & 34.20$\pm$ 6.90 & 38.41 & 28.76$\pm$ 5.42\\
  % + Two-Stage Joint Instruction Tuning 10 & 60.56 & 49.31 $\pm$ 11.65&& 46.37 & 33.29 $\pm$ 7.33 & 38.28 & 27.83 $\pm$ 5.86 \\
  \bottomrule
  \end{tabular}}
  % }
  \caption{\textbf{Zero-shot Performance on Miscellaneous.} The best performance is in \textbf{bold}.}
  \label{table:zs_vte}
  \end{table*}



\begin{table*}[!t]
  \centering
  \resizebox{0.91\linewidth}{!}{%
  % \tiny
  \begin{tabular}{l cc c cccc c cc}
  \toprule
   \multirow{3}{*}{\centering \textbf{Model}} & \multicolumn{2}{c}{\textbf{Visual Text Extraction}} && \multicolumn{4}{c}{\textbf{Visual Dialogue}} && \multicolumn{2}{c}{\textbf{Disaster Type Classification}} \\
   %
   \cline{2-3} \cline{5-8} \cline{10-11}
  %
  & \multicolumn{2}{c}{RougeL} && \multicolumn{2}{c}{RougeL} & \multicolumn{2}{c}{ACC} && \multicolumn{2}{c}{ACC}  \\
  \cline{2-3} \cline{5-8} \cline{10-11}
  & Max & Avg$\pm$ \text{Std} && Max & Avg $\pm$ \text{Std} & Max & Avg $\pm$ \text{Std} && Max & Avg $\pm$ \text{Std}  \\
  \midrule
  %\rowcolor{Gray} \multicolumn{8}{l}{\textbf{Baselines}} \\
  OFA & 36.31 & 17.62 $\pm$ 16.82 && 45.46 & 28.71 $\pm$ 9.81 & 37.63 & 23.97 $\pm$ 8.05 && 14.30 & 9.64 $\pm$ 4.34 \\
  OFA$_\text{TaskName}$ & 36.30 & - && 25.18 & - & 21.46 & - && 62.65 & -\\
OFA$_\text{MultiInstruct}$ & \textbf{74.35} & \textbf{62.43} $\pm$11.56 && \textbf{46.38}&32.91 $\pm$7.59 & \textbf{38.28} & 27.36 $\pm$ 6.17 && 64.88 &56.00 $\pm$12.96\\
\midrule
\rowcolor{Gray} \multicolumn{11}{l}{\textbf{Transfer Learning from \textsc{Natural Instructions}}} \\
OFA$_\text{NaturalInstruct}$ & 5.65 & 1.24 $\pm$ 2.48 && 30.94 & 27.91 $\pm$ 2.16 & 25.95 & 23.23 $\pm$ 1.92 && 56.64 & 38.21 $\pm$ 15.35  \\
OFA$_\text{MixedInstruct}$ & 62.43 & 46.56 $\pm$ 14.92 && 46.08 & \textbf{38.02} $\pm$ 5.25 & 37.98 & \textbf{31.58} $\pm$ 4.21 && \textbf{68.31} & \textbf{64.31} $\pm$ 2.39 \\
OFA$_\text{SeqInstruct}$ & 71.63 & 60.62 $\pm$ 12.31 && 46.17 & 35.10 $\pm$ 6.92 &38.11 & 29.10 $\pm$ 5.68 && 64.46 & 57.89 $\pm$ 9.51 \\
% OFA$_\text{AdapterInstruct}$ & \\
  \bottomrule
  \end{tabular}}
  % }
  \vspace{-2mm}
  \caption{\textbf{Zero-shot Performance on Miscellaneous.} The best performance is in \textbf{bold}.}
  \label{table:zs_vte}
  \vspace{-4mm}
  \end{table*}
